Estimation of Evaporator Valve Sizes in Supermarket Refrigeration Cabinets

In many applications, e.g. fault diagnostics and optimized control of supermarket refrigeration systems, it is important to determine the heat demand of the cabinets. This can easily be achieved by measuring the mass flow through each cabinet, however, that is expensive and not feasible in large-scale deployments. Therefore it is important to be able to estimate the valve sizes from the monitoring data, which is typically measured. The valve size is measured by an area, which can be used to calculate mass flow through the valve -- this estimated value is referred to as the valve constant. A novel method for estimating the cabinet evaporator valve constants is proposed in the present paper. It is demonstrated using monitoring data from a refrigeration system in a supermarket consisting of data sampled at a one-minute sampling rate, however it is shown that a sampling time of around 10-20 minutes is adequate for the method. Through thermodynamic analysis of a two-stage CO2 refrigeration system, a linear regression model for estimating valve constants was developed using time series data. The linear regression requires that transient dynamics are not present in the data, which depends on multiple factors e.g. the sampling time. If dynamics are not modeled it can be detected by a significant auto-correlation of the residuals. In order to include the dynamics in the model, an Auto-Regressive Moving Average model with eXogenous variables (ARMAX) was applied, and it is shown how it effectively eliminates the auto-correlation and provides more unbiased estimates, as well as improved the accuracy estimates. Furthermore, it is shown that the sample time has a huge impact on the valve estimates. Thus, a method for selecting the optimal sampling time is introduced. It works individually for each of the evaporators, by exploring their respective frequency spectrum.

==> Chapters/Introduction2.tex <==
\section{Introduction}
To take advantage of system modeling and automation, data-driven models and optimization are increasingly evolving [1] [2] [3] [4]. With the increasing amount and resolution of data being collected from all kinds of sources, the potential and applications are expanded, opening up new research questions to be answered.
Grey box modeling -- characterized by being a combination of white-box (physically based models) and black-box (purely data-driven models) -- of supermarket refrigeration systems is a research area of great interest and potential, both in optimized control and fault detection.  Thus, we achieve physical insight of the parameters of the overall and complex system using data points, [2] [5] [6] [7]. The method has been well tested in many applications, see i.a. [4] [8] - including refrigeration systems.
A promising approach to data-driven modeling and optimization of refrigeration systems is with neural networks and predictive control presented in [10] to increase the efficiency of the compressor in a refrigeration system. This is later shown in [11], where an energy reduction of 17\% was achieved. However, supermarkets' refrigeration systems are usually two-stage systems with two temperature levels, one for frozen goods and one for refrigerated goods, each with its own compressor equipment, which significantly complicates the models.

Data-driven modeling of supermarket refrigeration systems can be performed by modeling individual components; compressor, condenser or evaporator separately [12] [13] [14] - or the system can be modeled as an almost complete multi-component system [15] [16] [17]. Detailed data-driven models of a complete system were developed in [18] using subspace models - a method for parameterization in non-linear Multiple Input Multiple Output (MIMO) systems [19]. For single component models the parameterization can be done with a higher degree of detail, as it has fewer parameters per model compared to a single multi-component model - it makes parameter estimation much easier. A smart way to apply both principles is therefore first to parameterize separate models of the main components (e.g. evaporators, compressors and condenser) - this is done in [20] using of Predictive Error Minimization for parameterization. Afterwards, the complete system was modeled using the estimated parameters. In a simulation study, the model was used to develop management strategies that utilize the high heat capacity of the goods for flexible consumption in the electricity market and integrate supermarket refrigeration systems in smart-grid systems.
The models can give good predictions, but there is no guarantee that the estimated parameters are reasonable from a physical perspective. It is quite often the case that there are too many parameters to estimate, so that the models become over-parameterized and practically unidentifiable. In the modeling of the refrigeration system in [20] this is the case - the model can predict the temperature, which is the only thing needed for reliable control. However, if the parameter estimates are not physically correct, the properties and energy demand of the system are not known.
The problem with many previously proposed models is their lack of practicality due to high complexity. In [Grey Box Paper], this issue is addressed, arguing that simpler models may be necessary for real life scenarios. It also addresses an issue related to constantly changing parameters in the system model due to varying amounts of goods on store. Here, the constant related to the valve (the valve constant) is fixed (known from experimenting) – this also improves robustness and reliability of parameter estimates. The problem is that the valves will be unknown for automatic data driven modeling on a large scale.
Therefore, the present paper focuses on estimating these valve constants using a data driven approach. Two methods are presented for estimating the valve constants of a refrigeration system. First an estimation method where knowledge of the compressor stroke volume is required - here, a mass balance is formulated and a linear regression method is used to estimate the valve constants. For the second method, we have no knowledge of the compressor stroke volume - here a novel algorithm is presented, using prior knowledge of the different valve sizes that can possibly be installed to estimate the stroke volume, k-means clustering and an optimization algorithm. Finally, a residual model is applied for estimation of the valve sizes much in line with those estimated in the first method. This opens up for a fully automatized method for modelling supermarket refrigeration systems on a large scale with limited access to system data for individual supermarkets.


==> Chapters/Methodology2.tex <==
\section{The system}
The refrigeration system under study is illustrated in Figure \ref{fig:System}. Temperature and pressure measurements are accessible at all numbered points on the figure. After the receiver, at stage "1", the refrigerant is liquefied and split into the medium temperature (MT) string and the low temperature (LT) string, where expansion valves drops the pressure to the desired saturation temperature. The evaporators are controlled with valves using either hysteresis (open/close) or modulus (continues open) control - valve $i$ has a corresponding valve constant, denoted $A_i$. After the evaporators at stage "3a" and "3b", the refrigerant is super heated to avoid any droplets from entering the compressor. At stage "4a", "4b" and "5", after the low pressure compressor rack, the pressure is the same, but the enthalpy varies as the MT string and bypass (bp) string from the receiver connects. The refrigerant now enters the high pressure compressor rack and continues through the the condenser to a sub-cooled state at stage "8" - and the cycle repeats.

This research focus on modelling the evaporators, hence anything between stage "6" and "8" will not be discussed further. 

\begin{figure}
	\centering
		\includegraphics[scale=.2]{Figures/system_diagram.png}
	\caption{Exemplifying flow sheet of supermarket CO\textsubscript{2} refrigeration system. The valve constant for evaporator $i$ is denoted with $A_i$. $n_{\text{MT}}$ and $n_{\text{LT}}$ are the number of Medium -and Low Temperature evaporators respectively. }
	\label{fig:System}
\end{figure}



\section{Methodology}

\subsection{Method 1 - Valve estimation with known $V_s$}
The valve constants are used to determine the refrigerant mass flow through the evaporator $i$ from
\begin{align}
    \dot{m}_{\text{cab},i} = \sqrt{(P_{\text{rec}} - P_{e,i} ) \rho_{\text{liquid}}  } \lambda_i A_i ,
\end{align}
where $P_\text{rec}$ is the receiver pressure, $P_{\text{e},i}$ is the evaporator pressure for cabinet $i$, $\rho_{\text{liquid}}$ is the density of the liquefied refrigerant and $A$ is the valve constant. The opening degree of the valve of cabinet $i$, $\lambda_i$, is a number between 0 and 1 and is controlled either using hysteresis (open/close) or modular (continues open) control - this control parameter is highly correlated with the power load of the compressors - which of course links to the mass flow through the compressors. This mass flow can be expressed as
\begin{align}\label{eq:mass_comp}
    \dot{m} = \text{CAP} \eta_{\text{vol}} \cdot V_s \rho_{gas},
\end{align}
where $\eta_{\text{vol}, LT} \sim 0.8 $ and $\eta_{\text{vol}, MT} \sim 0.9 $. The displacement volume, $V_s$, can be obtained from the compressor information plate. From the overview in Figure \ref{fig:System}, it is clear that 
\begin{align}\label{eq:mass_LT}
    \dot{m}_{\text{LT,comp}} = \sum_{i=1}^{n_{\text{LT}}} \dot{m}_{\text{i}} = \sum_{i=1}^{n_{\text{LT}}} x_i A_i ,
\end{align}
where $n_{\text{LT}}$ is the total number of LT cabinets and $$x =  \sqrt{(P_{\text{rec}} - P_e ) \rho_{\text{liquid}}} \lambda $$
 For the MT cabinets,  we can setup the following mass balance
\begin{align}
    \dot{m}_{\text{MT,comp}} - \dot{m}_{\text{LT,comp}} - \dot{m}_{\text{bp}} = \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} \dot{m}_{i} = \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} x_{i} A_i ,
\end{align}
where $n_{\text{MT}}$ is the number of MT cabinets. We can calculate the mass flow from the by-pass valve as
\begin{align}
    \dot{m}_{\text{bp}} = Q(h_{\text{gc}}, P_{\text{rec}})\cdot \dot{m}_{\text{MT,comp}},
\end{align}

where $Q$ is the gas quality of the refrigerant from the by-pass valve as a function of the enthalpy in the gas cooler, $h_{\text{gc}}$, and the receiver pressure $P_\text{rec}$. This can be combined to the expression
\begin{align}\label{eq:mass_MT}
    \dot{m}_{\text{MT,comp}} (1- Q(h_{\text{gc}}, P_{\text{rec}})) - \dot{m}_{\text{LT,comp}} &= \sum_{i=n_{\text{LT}+1} 1}^{n_{\text{MT}}} x_i A_i ,
\end{align}

%\begin{figure}
%	\centering
%		\includegraphics[scale=.2]{Figures/od_cor_pow.png}
%	\caption{Opening degree of the  }
%	\label{fig:correlation_power}
%\end{figure}

Furthermore, by substituting Equation \ref{eq:mass_LT} into Equation \ref{eq:mass_MT}, the need for calculating the $\dot{m}_{\text{LT,comp}}$ is eliminated and it simplifies to

\begin{align}\label{eq:final}
    \dot{m}_{\text{MT,comp}} (1- Q(h_{gc}, P_{\text{rec}})) &= \sum_{i=1}^{n_{\text{MT}}} x_i A_i + \sum_{i=n_{\text{MT}} + 1}^{n_{\text{LT}}} x_i A_i\nonumber 
\end{align}.

Let $ y_t = \dot{m}_{\text{MT, comp},t} (1- Q(h_{\text{gc},t}, P_\text{rec},t)) $, then 
\begin{align}
    \boldsymbol{y} &= \begin{bmatrix}
                        y_{1} & y_{2} &  y_{n}
                    \end{bmatrix} \nonumber \\
    \boldsymbol{X} &= \begin{bmatrix}
                        x_{1,1} & x_{2,1} &  x_{n_V,1} \\
                        x_{1,2} & x_{2,2} & x_{n_V,2}\\
                        x_{1,n} & x_{2,n} & x_{n_V,n} 
                    \end{bmatrix}\nonumber \\
    \boldsymbol{\beta} &= \begin{bmatrix}
                        A_{1} & A_{2} &  A_{n_V} 
                    \end{bmatrix} \nonumber 
\end{align}
,
where $n$ is the number of observations and $n_V = n_{\text{MT}} + n_{\text{LT}}$.
 
And finally, we can write the linear regression model:
\begin{align}
    \boldsymbol{y} &= \boldsymbol{X}\boldsymbol{\beta} + \boldsymbol{\epsilon}, \\
    \text{for} \; \boldsymbol{\epsilon} &\sim N(0,\sigma^2 I) \; \text{and i.i.d},  \nonumber
\end{align}

Then $\boldsymbol{\beta}$ can be estimated from the least square regression that minimize:
\begin{align}
S(\boldsymbol{\beta}) =  ||\boldsymbol{y} - \boldsymbol{X}\boldsymbol{\beta}||^2 
\end{align}
and we obtain the ordinary least-squares solution
\begin{align}
\boldsymbol{\beta} = (\boldsymbol{X}^T \boldsymbol{X})^{-1} \boldsymbol{X}^T \boldsymbol{y}.\label{eq:ols}
\end{align}

% Since the outdoor temperature affects the efficiency of refrigeration systems, it can be beneficial to implement that into the model, e.g. $\boldsymbol{\beta} = [A_1,...,A_{n_V}, A_{T}]$, where $A_{T}$ is the coefficient for the temperature. % Furthermore, it is expected that operation during the day will lead to larger errors due to disturbances. 
\begin{figure*}[t]
	\centering
		\includegraphics[scale=.4]{Figures/optim.png}
	\caption{Optimization function}
	\label{fig:algorithm}
\end{figure*}
\subsection{Part 2 - Valve estimation with $V_{\text{s}}$ unknown} \label{sec:unknown_v}

The compressor stroke volume, $V_{\text{s}}$, is not always easily accessible thus for automatic implementation on a large scale, a valve estimation methodology with $V_s$ unknown is required. With knowledge about the types of valves there possibly can be in the system - see Table \ref{tab:danfoss_valves} in Appendix \ref{Appendix:Actual_valve_sizes} - a novel algorithm was developed, using K-means for clustering the estimated valve constants $\mathbf{A}$. Figure \ref{fig:algorithm} illustrates part of the algorithm. 

\begin{itemize}
    \item We have a function with two inputs:
    \begin{itemize}
        \item The MT compressor stroke volume $V_{\text{s}}$
        \item An initial guess of the different types of valve we have in the system - we call that $a$.
    \end{itemize}
    \item First we estimate the model coefficients, $\hat{\boldsymbol{\beta}}$, from Equation \ref{eq:ols}.  
    \item Then we apply k-means to $ \hat{\boldsymbol{\beta}}$ e.g. each $\hat{\beta}_i$ is assigned to cluster $S_i$ by minimizing:
    
    $$
    \argmin_S \sum_{i=1}^k \sum_{\boldsymbol{x} \in S_i} \norm{\boldsymbol{x} - \boldsymbol{C_i}}^2,
    $$
    where $\boldsymbol{C_i}$ is the mean of cluster $i$:
    \begin{align}
    C_i = \frac{1}{S_i^{(t)}} \sum_{A_j \in S_i^{(t)}} A_j
    \end{align}
\end{itemize}

% $f(V_{\text{s}})$ refers to Equation \ref{eq:final}, where  $\dot{m}_{MT}$ is a function of $V_s$ (see Eq. \ref{eq:mass_comp}). The illustration is a function with two inputs; the compressor stroke volume, $V_s$, and an initial guess of $\mathbf{a}$ (the kind of valves that exist in the system). The output is a Root Mean Squared Error of $\epsilon$. 
%First, we will get an estimate of the valve constants $\mathbf{A}$ from $f(V_s)$. Then we apply k-means to $\mathbf{A}$ e.g. each $A_i$ is assigned to cluster $S_i$ as:
%\begin{align}
%    S_i^{(t)} = A_p : \norm{A_p - C_i^{(t)} }^2 \leq \norm{A_p - C_j^{(t)} }^2 \;\; \forall, 1 \leq j \leq k
%\end{align}
%where $k$ is the number of valve constants in $\mathbf{a}$ and $\mathbf{C}$ is the cluster means:





$\boldsymbol{C}$ and $\boldsymbol{a}$ are sorted vectors from smallest to largest so that we get the error
$
    \epsilon_1 = \ln{\boldsymbol{C}} - \ln{\boldsymbol{a}}
$. 
At last, we get the Root Mean Squared Error output of the function, referred to as $E_1$:
\begin{align}\label{eq:E_1}
    E_1 = \frac{\sqrt{\sum_{i=1}^{N_{\epsilon_1}} \epsilon_{1,i}^2}}{N_{\epsilon_1}},
\end{align}
where $N_{\epsilon}$ is the length of $\epsilon$.

For the optimization, we assume $\boldsymbol{a}$ is known and use the one dimensional "Brent" optimization algorithm to find the $V_{\text{s}}$ that minimizes the $E_1$.
With 7 different types of valves, we have 127 different combinations of $\boldsymbol{a}$ thus the above algorithm is not enough on its own. By running the algorithm on all the combinations, we can investigate the errors and pick out the combination that produces the best model. For the error estimates, we use $E_1$ and the following:
\begin{align}\label{eq:E_2}
    E_2 = \frac{1}{n_V} \sum_{i=1}^k \sum_{\hat{\beta}_j \in S_i} (\ln{C_i} - \ln{\hat{\beta}_j})^2,
\end{align}
%where
%\begin{align}
%    \epsilon_{2,j} =   \ln{C_i} -  \ln{A_j}; \quad  A_j \in S_i^{(t)}\nonumber
%\end{align}

$E_2$ is thus the cluster uncertainty of $\boldsymbol{C}$.

% Furthermore, we are interested in a normally distributed $E_1$, which can be indicated by the skewness:

%\begin{align}
%    \text{Skewness} &= 3*(C_{E_1} - \text{median}_{E_1}) / \sigma_{E_1} \label{eq:skewness}
%\end{align}
%A large skewness means that at least one of the estimates in $\mathbf{C}$ stands out from the rest, indicating one too many or one too few valves in $a$.
%A last criteria is the correlation between $\mathbf{C}$ and $ \mathbf{a}$:
%\begin{align}
%    \rho &=     \frac{\text{cov}(\ln{\mathbf{C}} , \ln{\mathbf{a}})}{\sigma_C \sigma_a}. \label{eq:rho}
%\end{align}

%The closer $\rho$ is to 1, the more correct are the internal "jumps" between the valve sizes e.g. $a_j - a_i$ is similar to $C_j - C_i$. 




\subsection{Data}the data stretch approximately eight months from November 2013 to June 2014
The data is available in 1 minute values stretching approximately eight months from November 2013 to June 2014 and is illustrated for one cabinet during one night in Figure \ref{fig:night} (left plot). If we use the raw 1-minute data, we will experience a lot of redundant noise that will lead to a bad model with auto correlation. Thus we need to find the best data resolution for the model. One way is to find the lowest resolution that removes all significant auto-correlation from the model. In this case, 20 minute data is found to be the optimal resolution.

 


\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{Figures/night_operation.pdf}
    \caption{left plot: $x$ of cabinet 20A (freezing room) the 26th of October 2013. Right plot: The frequency spectrum for 20A.}
    \label{fig:night}
\end{figure*}


\begin{figure*}[t]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/timeseries.png}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/timeseries2.png}
  \end{minipage}
  \caption{Daily averages of the mass flow through the MT evaporators, $\mathbf{Y}$, and $\mathbf{X}$ for all the cabinets.}\label{fig:timeseries}
\end{figure*}


%From Equation \ref{eq:mass_MT}, it is claimed that the variable $\boldsymbol{X}$ is correlated to the mass flow from the MT evaporators. This is confirmed in Figure \ref{fig:corr_plot} - the top line in the scheme shows the correlation between the mass flow and $x$ for each cabinet. The color indicates the size of the valve - the darker the blue the larger the valve. This genuinely tends to hold true according to actual valve constants - see Appendix \ref{Appendix:Actual_valve_sizes}. 
Some of the cabinets are connected on the same string e.g. 40A, 40B and 40C - see Appendix \ref{Appendix:structure} for the cabinet structure. The operation of these cabinets is therefore quite similar and correlation might occur - this can be crucial for the model, as this can lead to co-linearity. When this happens the condition number of the matrix $\mathbf{X}$ is lowered, making the determinant of it close to zero, and thus inverting it results in large numerical errors - see Equation \ref{eq:ols}. However, in this case co-linearity is not an issue (generally, a correlation coefficient $>0.7$ indicates co-linearity \cite{Dormann} ). To confirm further, the Variance Inflation Factor (VIF) is a widely uesd tool - a variant of stepwise regression used to detect multi co-linearity. A VIF less than 10 is an acceptable level \cite{Hair} - in this case, the VIF is less than 2.


\begin{figure}
	\centering
		\includegraphics[scale=0.5]{Figures/cor_valves.pdf}
	\caption{Pearson correlation plot of $\boldsymbol{X}$ and the mass flow from the MT evaporators}
	\label{fig:corr_plot}
\end{figure}



==> Figures/model.tex <==
%% Scaling the nodes
\tikzset{every node/.style={scale=\scaleTikz}}
%% The tikz
\begin{circuitikz}[xscale=\scaleTikz, yscale=\scaleTikz]
  %% Define variables to control size
  \def\x{2.3}    % x distance between nodes
  \def\y{3.3}    % y position of the diagram
  \def\ylab{4} % y position of the labels
  %% Set the coordinates
 \coordinate (Goods) at (0,0);
 \coordinate (R_goods) at ($(Goods)+(\x,0)$);
 \coordinate (Cabinet) at ($(R_goods)+(\x,0)$);
 \coordinate (R_c) at ($(Cabinet)+(\x,0)$);

 
 
 
  \coordinate (Floor) at (0,0);
  \coordinate (Heater) at ($(Floor)+(0.8*\x,0)$);
  \coordinate (SolarFloor) at ($(Heater)+(\x,0)$);
  \coordinate (Interior) at ($(SolarFloor)+(\x,0)$);
  \coordinate (SolarInterior) at ($(Interior)+(1.3*\x,0)$);
  %\coordinate (HeaterInterior) at ($(Interior)+(\x,0)$);
  \coordinate (WallLeft) at ($(SolarInterior)+(0.45*\x,0)$);
  \coordinate (Wall) at ($(WallLeft)+(0.8*\x,0)$);
  \coordinate (WallRight) at ($(Wall)+(0.8*\x,0)$);
  \coordinate (Ambient) at ($(WallRight)+(0.25*\x,0)$);
  %% Draw stuff
  \draw
  ($(3.15*\x,0)$) node[ground] {}
  % ($(6.15*\x,0)$) node[ground] {}

 % ($(Floor)+(0,4.5)$) -- ($(SolarFloor)+(0,4.5)$)
 % ($(Floor)+(0,6)$) -- ($(SolarFloor)+(0,6)$)
 
  %($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1)$)
  %($(Heater)+(\xoffset,1)$) to[I, l=$\Ph$] %($(Heater)+(\xoffset,\y)$);
 
  (Goods) -- (Ambient) % The bottom line
  %%($(Floor)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  ($(Goods)+(0,\y)$) -- ($(R_goods)+(0,\y)$) % The top line
   ($(Cabinet)+(0,\y)$) -- ($(R_c)+(0,\y)$); % The top line
%%($(R_c)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  % The top line

  %% The Floor
 \draw
  (Goods) to[C=$\Cg$, -*] ($(Goods)+(0,\y)$)
  {[anchor=south east] ($(Goods)+(0.2,\y)$) node {$\Tg$}};
  %% The Heater
%%  \def\xoffset{-0.25*\x}
%%  \draw
%%  ($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1.2)$)
%%  ($(Heater)+(\xoffset,1.2)$) to[I, l_=$(1-\Psi\n{h})\Ph$] %%($(Heater)+(\xoffset,\y)$);
  
  %% The Solar to floor
 %% \def\xoffset{0.1*\x}
 %% \draw
 %% ($(SolarFloor)+(\xoffset,0)$) to[I, l=$(1-\Psi\n{s}) %%\gA\Ps$]($(SolarFloor)+(\xoffset,\y-1.2)$)
 %% ($(SolarFloor)+(\xoffset,\y-1.2)$) -- %%($(SolarFloor)+(\xoffset,\y)$);
  %% Resistance
  \draw
  ($(R_goods)+(0,\y)$) to [R, l=$\Rg$] ($(Cabinet)+(0,\y)$);
  %% The Interior
  \draw
  (Cabinet) to[C=$\Cc$, -*] ($(Cabinet)+(0,\y)$)
  {[anchor=south east] ($(Cabinet)+(0.2,\y)$) node {$\Tc$}};
 \draw
  ($(R_c)+(0,\y)$) to [R, l=$\Rload$] ($(Ambient)+(0,\y)$);


  %% The Solar to interior
  \def\xoffset{0.1*\x}
  \draw
  %%($(Heater)+(\xoffset+5.5,0)$) -- ($(Heater)+(\xoffset+5.5,0.2)$)
  ($(Heater)+(\xoffset+5.5,0)$)
  to[I, l_=$ \frac{1}{\Rm } \Mr (\Tc-\Te)$] ($(Heater)+(\xoffset+5.5,\y)$);
  

%%  \def\xoffset{0*\x}
 %% \draw
 %% ($(SolarInterior)+(\xoffset+0.5,0)$) to[I, %%l=$\Psi\n{s}\gA\Ps$]($(SolarInterior)+(\xoffset+0.5,\y-1.2)$)
%%  ($(SolarInterior)+(\xoffset+0.5,\y-1.2)$) -- ($(SolarInterior)+(\xoffset+0.5,\y)$);
  %% The Wall
  %%\draw
 %% ($(WallLeft)+(0,\y)$) to [R, l=$\Riw$, -*] ($(Wall)+(0,\y)$)        
 %% ($(Wall)+(0,\y)$) to [R, l=$\Rwa$] ($(WallRight)+(0,\y)$)
 %% ($(WallRight)+(0,\y)$) -- ($(Ambient)+(0,\y)$)
 %% (Wall) to[C=$\Cw$, -] ($(Wall)+(0,\y)$)
 %% {[anchor=south east] ($(Wall)+(0.2,\y)$) node {$\Tw$}};
  %% The Ambient
  \draw
  [V, l=$\Ta$] ($(Ambient)+(0,\y)$) to ($(Ambient)+(0,0)$);
  %% The dashed lines
 %% \def\xoffset{0.22*\x}
 %% \draw
 %% [dashed] ($(SolarFloor)+(\xoffset*\x,-0.5)$) -- %%($(SolarFloor)+(\xoffset*\x,\y-0.4)$)  
%%  [dashed] ($(SolarFloor)+(\xoffset*\x,\ylab+0.2)$) -- ($(SolarFloor)+(\xoffset*\x,\ylab+1)$)  
%%  [dashed] ($(WallLeft)+(0.15,-0.5)$) -- ($(WallLeft)+(0.15,\ylab+1)$)  
%%  [dashed] ($(Ambient)+(-0.3*\x,-0.5)$) -- ($(Ambient)+(-0.3*\x,\ylab+1)$);
  %% The labels
 %% \draw
%%  {[anchor=south] ($(Heater)+(0.2,\ylab)$) node{\Large Floor}}
%%  {[anchor=south] ($(Interior)+(0.7*\x,\ylab)$) node{\Large Interior}}
%%  {[anchor=south] ($(Wall)+(0,\ylab)$) node{\Large Envelope}}
 %% {[anchor=south] ($(Ambient)+(0.2*\x,\ylab)$) node{\Large Ambient}};

\end{circuitikz}


==> Figures/model_simple.tex <==
%% Scaling the nodes
\tikzset{every node/.style={scale=\scaleTikz}}
%% The tikz
\begin{circuitikz}[xscale=\scaleTikz, yscale=\scaleTikz]
  %% Define variables to control size
  \def\x{2.3}    % x distance between nodes
  \def\y{3.3}    % y position of the diagram
  \def\ylab{4} % y position of the labels
  %% Set the coordinates
 \coordinate (Goods) at (0,0);
 \coordinate (R_goods) at ($(Goods)+(\x,0)$);
 \coordinate (Cabinet) at ($(R_goods)+(\x,0)$);
 \coordinate (R_c) at ($(Cabinet)+(\x,0)$);

 
 
 
  \coordinate (Floor) at (0,0);
  \coordinate (Heater) at ($(Floor)+(0.8*\x,0)$);
  \coordinate (SolarFloor) at ($(Heater)+(\x,0)$);
  \coordinate (Interior) at ($(SolarFloor)+(\x,0)$);
  \coordinate (SolarInterior) at ($(Interior)+(1.3*\x,0)$);
  %\coordinate (HeaterInterior) at ($(Interior)+(\x,0)$);
  \coordinate (WallLeft) at ($(SolarInterior)+(0.45*\x,0)$);
  \coordinate (Wall) at ($(WallLeft)+(0.8*\x,0)$);
  \coordinate (WallRight) at ($(Wall)+(0.8*\x,0)$);
  \coordinate (Ambient) at ($(WallRight)+(0.25*\x,0)$);
  %% Draw stuff
  \draw
  ($(3.15*\x,0)$) node[ground] {}
  % ($(6.15*\x,0)$) node[ground] {}

 % ($(Floor)+(0,4.5)$) -- ($(SolarFloor)+(0,4.5)$)
 % ($(Floor)+(0,6)$) -- ($(SolarFloor)+(0,6)$)
 
  %($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1)$)
  %($(Heater)+(\xoffset,1)$) to[I, l=$\Ph$] %($(Heater)+(\xoffset,\y)$);
 
  (Cabinet) -- (Ambient) % The bottom line
  %%($(Floor)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  %%($(Goods)+(0,\y)$) -- ($(R_goods)+(0,\y)$) % The top line
   ($(Cabinet)+(0,\y)$) -- ($(R_c)+(0,\y)$); % The top line
%%($(R_c)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  % The top line

  %% The Floor
%% \draw
%%  (Goods) to[C=$\Cg$, -*] ($(Goods)+(0,\y)$)
%%  {[anchor=south east] ($(Goods)+(0.2,\y)$) node {$\Tg$}};
  %% The Heater
%%  \def\xoffset{-0.25*\x}
%%  \draw
%%  ($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1.2)$)
%%  ($(Heater)+(\xoffset,1.2)$) to[I, l_=$(1-\Psi\n{h})\Ph$] %%($(Heater)+(\xoffset,\y)$);
  
  %% The Solar to floor
 %% \def\xoffset{0.1*\x}
 %% \draw
 %% ($(SolarFloor)+(\xoffset,0)$) to[I, l=$(1-\Psi\n{s}) %%\gA\Ps$]($(SolarFloor)+(\xoffset,\y-1.2)$)
 %% ($(SolarFloor)+(\xoffset,\y-1.2)$) -- %%($(SolarFloor)+(\xoffset,\y)$);
  %% Resistance
 %% \draw
%%  ($(R_goods)+(0,\y)$) to [R, l=$\Rg$] ($(Cabinet)+(0,\y)$);
  %% The Interior
  \draw
  (Cabinet) to[C=$\Cc$, -*] ($(Cabinet)+(0,\y)$)
  {[anchor=south east] ($(Cabinet)+(0.2,\y)$) node {$\Tc$}};
 \draw
  ($(R_c)+(0,\y)$) to [R, l=$\Rload$] ($(Ambient)+(0,\y)$);


  %% The Solar to interior
  \def\xoffset{0.1*\x}
  \draw
  %%($(Heater)+(\xoffset+5.5,0)$) -- ($(Heater)+(\xoffset+5.5,0.2)$)
  ($(Heater)+(\xoffset+5.5,0)$)
  to[I, l_=$ \frac{1}{\Rm }\Mr (\Tc-\Te)$] ($(Heater)+(\xoffset+5.5,\y)$);
  

%%  \def\xoffset{0*\x}
 %% \draw
 %% ($(SolarInterior)+(\xoffset+0.5,0)$) to[I, %%l=$\Psi\n{s}\gA\Ps$]($(SolarInterior)+(\xoffset+0.5,\y-1.2)$)
%%  ($(SolarInterior)+(\xoffset+0.5,\y-1.2)$) -- ($(SolarInterior)+(\xoffset+0.5,\y)$);
  %% The Wall
  %%\draw
 %% ($(WallLeft)+(0,\y)$) to [R, l=$\Riw$, -*] ($(Wall)+(0,\y)$)        
 %% ($(Wall)+(0,\y)$) to [R, l=$\Rwa$] ($(WallRight)+(0,\y)$)
 %% ($(WallRight)+(0,\y)$) -- ($(Ambient)+(0,\y)$)
 %% (Wall) to[C=$\Cw$, -] ($(Wall)+(0,\y)$)
 %% {[anchor=south east] ($(Wall)+(0.2,\y)$) node {$\Tw$}};
  %% The Ambient
  \draw
  [V, l=$\Ta$] ($(Ambient)+(0,\y)$) to ($(Ambient)+(0,0)$);
  %% The dashed lines
 %% \def\xoffset{0.22*\x}
 %% \draw
 %% [dashed] ($(SolarFloor)+(\xoffset*\x,-0.5)$) -- %%($(SolarFloor)+(\xoffset*\x,\y-0.4)$)  
%%  [dashed] ($(SolarFloor)+(\xoffset*\x,\ylab+0.2)$) -- ($(SolarFloor)+(\xoffset*\x,\ylab+1)$)  
%%  [dashed] ($(WallLeft)+(0.15,-0.5)$) -- ($(WallLeft)+(0.15,\ylab+1)$)  
%%  [dashed] ($(Ambient)+(-0.3*\x,-0.5)$) -- ($(Ambient)+(-0.3*\x,\ylab+1)$);
  %% The labels
 %% \draw
%%  {[anchor=south] ($(Heater)+(0.2,\ylab)$) node{\Large Floor}}
%%  {[anchor=south] ($(Interior)+(0.7*\x,\ylab)$) node{\Large Interior}}
%%  {[anchor=south] ($(Wall)+(0,\ylab)$) node{\Large Envelope}}
 %% {[anchor=south] ($(Ambient)+(0.2*\x,\ylab)$) node{\Large Ambient}};

\end{circuitikz}


==> Valve Estimation part 1 (1)/Chapters/Conclusion.tex <==
\section{Conclusion}

Models for estimating the valve constants in supermarket refrigeration systems are presented and results are obtained from data collected in a regular supermarket in Denmark. A mass balance is formulated leading to a linear regression model from which the valve constants can be estimated -- and it is extended to an ARMAX model, which can describe the system dynamics. The estimated results are analysed and it is shown that reliable values can be obtained, but that several factors must be taken into account. Firstly, co-linearity in the inputs can cause issues, but this is not an issue in the case study -- potentially it can be a problem for other systems, and should be checked e.g. with the Variance Inflation Factor. Furthermore, the coefficient estimates vary with the sampling time and it is shown that no single sampling time is optimal for all evaporators, because they have different cycle times. However, for models using sampling times above 15 min., the valve estimates become more stable and less dependent on the sampling time. Some variation is still found, hence some smoothing of the estimates as a function of the sampling time can be beneficial, however an approach to this must be developed with data from multiple supermarkets. The suggested approach for an optimal sampling time is shown to be a good indicator for the best estimates.
Auto-correlation is highly present in the linear regression models, thus to account for this, an ARMAX$_{4,1}$ is applied. After applying the ARMAX$_{4,1}$ model, the CI for the valve estimates becomes more narrow, suggesting a more accurate model. Furthermore, the estimates are also slightly less dependent on the sampling time than with the linear regression model. Thus it is found, that the ARMAX model is preferable over the linear regression model, however still studies including a wide range of supermarkets must be carried out to further develop the methodology and study its full potential.

==> Valve Estimation part 1 (1)/Chapters/Discussion.tex <==

\section{Discussion}

The method for valve estimation provides useful results, however, the sampling time turned out to have a huge impact which must be handled to achieve reliable estimates. An issue with the method is that the evaporators have very different optimal sampling times given their different frequencies. Thus, there exist no single sampling time suitable for all the evaporators. However, an approach for identifying an optimal sampling time for each evaporator was presented and is was shown that estimates, at their respective optimal sampling time, fits fairly well with the specified valve constants. Notice, for the linear regression model the optimal sampling time is at a point on the graphs (in Figure \ref{fig:res}), where the valve constant estimates either begin to converge, or they are found in a local optimum. For the ARMAX model, the sampling time is far less important -- the valve constant estimates do not vary much using sampling times above $10$ min.. However, we still see generally more accurate results around the optimal sampling time. These effects should be studied in further research including multiple supermarkets.

Models using sampling times below $10$ min. provided generally very different results and the residuals were also highly correlated (See Figure \ref{fig:acf} left plots for the 1 minute models) -- both in the linear regression model as well as the ARMAX$_{4,1}$ model. For models using sampling times $> 15$ min., the results were much more uniform in both the linear regression model and the ARMAX model. Problems with the residuals are however still present for the linear regression model -- these are fixed in the ARMAX$_{4,1}$ model. 

It is clear that the CIs are much more narrow for the ARMAX$_{4,1}$ models, suggesting a generally better model. The estimates for the ARMAX$_{4,1}$ models using a sampling time above $15$ min. are also less dependent on the sampling time than for the linear regression model. However, for the cabinet MT$_7$, there are still some rather large estimate variations. This is because the cabinet uses modulating control rather than hysteresis control as all the others use. Therefore, the more accurate valve constant estimates may be an average of the estimates from the ARMAX$_{4,1}$ models using sampling times between 15 and 20 min. to even out the variation. We may calculate an average of the estimates from models using sampling times around the optimal sampling time, if this exists. 

The method has only been tested on one refrigeration system with mixed controls -- one evaporator used modulating -- and the rest used hysteresis control. It will be interesting to expand the study to include supermarkets that only use modulating control and supermarkets that only use hysteresis control. Consistency among the evaporators is expected to give better results. 

This study used 8 months of data for the results -- it is, however, possible to calculate the estimates with less data, but the uncertainty will increase. As much data as possible should be used for the estimates, however, periods where faults have occurred should be removed to ensure right estimates.




==> Valve Estimation part 1 (1)/Chapters/Introduction.tex <==
\section{Introduction}
To take advantage of system modeling and automation, the use of digital twins (a digital representation of a physical system) are increasingly evolving \citep{Yuchen,BACHER20111511}. With the increasing amount and resolution of data being collected from all kinds of sources, the potential and applications are expanded, opening up new research questions to be answered. This paper focus specifically on estimation of evaporator valve constants (a measure of the valve area when fully opened) of the evaporators in supermarket refrigeration cabinets, to enable a better understanding of these systems on a large scale. Without correct valve constants, the energy demand for each evaporator cannot be determined without measuring the mass flow directly which is expensive and practically infeasible.

Grey box modeling -- characterized by being a combination of white-box (physically based models) and black-box (purely data-driven models) -- of supermarket refrigeration systems is a research area of great interest and potential. The models can be used in for applications in optimized control and fault detection.  Thus, we achieve physical insight of the parameters of the overall and complex system using measured time series data, \citep{MARUTA20131090,KRISTENSEN20041431}. The method has been well tested in many applications, see e.g. \citep{BROK2019494,KIM2018359} for  refrigeration systems applications.
A promising approach to data-driven modeling and optimization of refrigeration systems is with neural networks and predictive control presented in \citep{KIZILKAN201111686} to increase the efficiency of the compressor in a refrigeration system. This is later followed-up in \citep{pr8091106}, where an energy reduction of 17\% was achieved on a one-stage system. However, supermarkets' refrigeration systems are usually two-stage systems with two temperature levels, one for frozen goods and one for refrigerated goods, each with its own compressor equipment, which significantly complicates the models.

Data-driven modelling of supermarket refrigeration systems can be done by modelling single components; compressor, condenser or evaporator separately \citep{Perez,Cecchinato,Willatzen} -- or the system may be modelled as a near-complete refrigeration system with several components integrated \citep{Aprea,Wang,Zhou}. Detailed data-driven models of a complete system was developed in \citep{Glenn}, using sub-space models -- a method for model parameterization of non-linear Multiple Inlet Multiple Outlet (MIMO) systems \citep{Katayama}. In that work, the cooling cabinets were not considered individually. For single component models, the parameterization can be done in a higher detail and will have fewer parameters per model compared to multi-component model.
A clever way to use both principles, is to first parameterize separate models of the main components (e.g. cooling cabinets, compressors and the condenser) -- this is done in \citep{Ehsan}, using Predictive Error Minimization for parameter estimation. Afterwards the complete system was modelled using the estimated parameters. The model was used to develop control strategies for providing energy flexibility aiming to integrate supermarket refrigeration systems in smart grids. 
  \begin{figure}[t]
	\centering
		\includegraphics[scale=.2]{Figures/system_diagram.png}
	\caption{Exemplifying flow sheet of supermarket CO\textsubscript{2} refrigeration system. The valve constant for evaporator $i$ is denoted with $A_i$. The $n_{\text{MT}}$ and $n_{\text{LT}}$ are the number of Medium -and Low Temperature evaporators respectively. }
	\label{fig:System}
\end{figure}
Even though the models after parameter estimation may generate good predictions, there is no guarantee that the parameters are reasonable from a physical perspective. It is quite often the case that there are too many parameters to estimate, such that the models become over-parameterized and unidentifiable. In the modelling of cooling cabinets in \citep{Ehsan}, this is the case. The model can predict the temperature which is the only thing needed for control. However, if the parameters are not physically correct, we have no knowledge about the energy demand. 

The problem with many previously proposed models is their lack of practicality due to high complexity. In \cite{GreyBox}, this issue is addressed, arguing that simpler models are necessary for automatic large-scale deployment. Furthermore, the issue related to constantly changing parameters in the system model due to varying amounts of goods on store was addressed. Here, a fixed valve constant is used (known from specifications), the valve constants will in most cases be unknown for automatic large-scale deployment.
Therefore, the present paper focuses on estimating these valve constants using a data driven approach. % with data from AK-Centralen A/S\footnote{\url{www.ak-centralen.dk}}. 
First, a mass balance is formulated as a linear regression model -- with the valve constants being the model coefficients. Thus, the Ordinary Least Squares solution (OLS) is used to estimate the valve constants. Furthermore, a method for selecting the optimal sampling time is suggested and applied for each evaporator, it is based on their respective frequency spectrum.
One assumption which must hold for the linear regression model to provide unbiased estimates is that there are no transient dynamics in the modeled data. By analysing residuals it is found that they have a significant and high auto-correlation -- which means that the dynamics were not modeled. To account for this, an ARMAX (Auto Regressive Moving Average with eXogenous variables) model is applied for more accurate estimates of the valve constants.
The methods presented in this paper opens up for a fully automatized method for modelling supermarket refrigeration systems on a large scale with limited access to knowledge of the individual supermarkets, only monitoring data, which is typically available, is used.

\begin{comment}
This is essentially determined by the cabinet valve constant -- a measure of the specific evaporator valve size, varying from cabinet to cabinet. Therefore, it is very useful to know these valve constants thereby enabling a correct modelling of the energy demand from each cabinet. In the present paper, two methods are presented for estimating the valve constants of a refrigeration system. First an estimation method where knowledge of the compressor stroke volume is required -- here, a mass balance is formulated and a linear regression method is used to estimate the valve constants. For the second method, we have no knowledge of the compressor stroke volume -- here a novel algorithm is presented, using prior knowledge of the different valve sizes that can possibly be installed to estimate the stroke volume, k-means clustering and an optimization algorithm. Finally, a residual model is applied for estimation of the valve sizes much in line with those estimated in the first method. This opens up for a fully automatized method for modelling supermarket refrigeration systems on a large scale with limited access to system data for individual supermarkets.

Good models of the energy demand in supermarket refrigeration systems are of great importance in developing fault detection systems, cabinet categorization and energy optimization control strategies.
\end{comment}





==> Valve Estimation part 1 (1)/Chapters/Introduction2.tex <==
\section{Introduction}
To take advantage of system modeling and automation, data-driven models and optimization are increasingly evolving [1] [2] [3] [4]. With the increasing amount and resolution of data being collected from all kinds of sources, the potential and applications are expanded, opening up new research questions to be answered.
Grey box modeling -- characterized by being a combination of white-box (physically based models) and black-box (purely data-driven models) -- of supermarket refrigeration systems is a research area of great interest and potential, both in optimized control and fault detection.  Thus, we achieve physical insight of the parameters of the overall and complex system using data points, [2] [5] [6] [7]. The method has been well tested in many applications, see i.a. [4] [8] - including refrigeration systems.
A promising approach to data-driven modeling and optimization of refrigeration systems is with neural networks and predictive control presented in [10] to increase the efficiency of the compressor in a refrigeration system. This is later shown in [11], where an energy reduction of 17\% was achieved. However, supermarkets' refrigeration systems are usually two-stage systems with two temperature levels, one for frozen goods and one for refrigerated goods, each with its own compressor equipment, which significantly complicates the models.

Data-driven modeling of supermarket refrigeration systems can be performed by modeling individual components; compressor, condenser or evaporator separately [12] [13] [14] - or the system can be modeled as an almost complete multi-component system [15] [16] [17]. Detailed data-driven models of a complete system were developed in [18] using subspace models - a method for parameterization in non-linear Multiple Input Multiple Output (MIMO) systems [19]. For single component models the parameterization can be done with a higher degree of detail, as it has fewer parameters per model compared to a single multi-component model - it makes parameter estimation much easier. A smart way to apply both principles is therefore first to parameterize separate models of the main components (e.g. evaporators, compressors and condenser) - this is done in [20] using of Predictive Error Minimization for parameterization. Afterwards, the complete system was modeled using the estimated parameters. In a simulation study, the model was used to develop management strategies that utilize the high heat capacity of the goods for flexible consumption in the electricity market and integrate supermarket refrigeration systems in smart-grid systems.
The models can give good predictions, but there is no guarantee that the estimated parameters are reasonable from a physical perspective. It is quite often the case that there are too many parameters to estimate, so that the models become over-parameterized and practically unidentifiable. In the modeling of the refrigeration system in [20] this is the case - the model can predict the temperature, which is the only thing needed for reliable control. However, if the parameter estimates are not physically correct, the properties and energy demand of the system are not known.
The problem with many previously proposed models is their lack of practicality due to high complexity. In [Grey Box Paper], this issue is addressed, arguing that simpler models may be necessary for real life scenarios. It also addresses an issue related to constantly changing parameters in the system model due to varying amounts of goods on store. Here, the constant related to the valve (the valve constant) is fixed (known from experimenting) – this also improves robustness and reliability of parameter estimates. The problem is that the valves will be unknown for automatic data driven modeling on a large scale.
Therefore, the present paper focuses on estimating these valve constants using a data driven approach. Two methods are presented for estimating the valve constants of a refrigeration system. First an estimation method where knowledge of the compressor stroke volume is required - here, a mass balance is formulated and a linear regression method is used to estimate the valve constants. For the second method, we have no knowledge of the compressor stroke volume - here a novel algorithm is presented, using prior knowledge of the different valve sizes that can possibly be installed to estimate the stroke volume, k-means clustering and an optimization algorithm. Finally, a residual model is applied for estimation of the valve sizes much in line with those estimated in the first method. This opens up for a fully automatized method for modelling supermarket refrigeration systems on a large scale with limited access to system data for individual supermarkets.


==> Valve Estimation part 1 (1)/Chapters/Methodology.tex <==
\nomenclature[A]{$\dot{m}$}{Mass flow 
  \nomunit{$\text{kg}/\text{s}$}}
\nomenclature[A]{$P$}{Pressure
  \nomunit{Bar}}
\nomenclature[B]{rec}{Receiver
  \nomunit{}}
\nomenclature[B]{$e$}{Evaporator
  \nomunit{}}
\nomenclature[B]{liq}{Liquid phase
  \nomunit{}}
\nomenclature[A]{$\rho$}{Density
  \nomunit{kg/m$^3$}} 
 \nomenclature[A]{$\lambda$}{Opening degree (0-1)
  \nomunit{-}}
 \nomenclature[A]{$A$}{Valve constant
  \nomunit{$\sqrt{10}$ m$^2$}}
 \nomenclature[A]{$A$}{Valve constant
  \nomunit{$\sqrt{10}$ m$^2$}}
 \nomenclature[A]{f}{Virtual compressor frequency (load as percentage of maximum capacity 0-1)
  \nomunit{$-$}}
\nomenclature[A]{$\eta_{\text{vol}}$}{Volumetric efficiency (0-1)
  \nomunit{$-$}}
 \nomenclature[A]{$V_\text{s}$}{Compressor stroke volume
  \nomunit{m$^3$}}
 \nomenclature[B]{gas}{Gas phase
  \nomunit{}}  
 \nomenclature[A]{$Q$}{Gas quality (0-1)
  \nomunit{-}}  
  \nomenclature[A]{$h$}{Enthalpy
  \nomunit{J/kg}} 
 \nomenclature[B]{LT}{Low temperature
  \nomunit{}} 
 \nomenclature[B]{MT}{Medium temperature
  \nomunit{}}
  \nomenclature[B]{comp}{Compressor rack
  \nomunit{}}
  \nomenclature[B]{gc}{Gas cooler
  \nomunit{}}
  


\section{The system}
The refrigeration system under study is illustrated in Figure \ref{fig:System}. Temperature and pressure measurements are accessible at all numbered points on the figure. The process is the following. After the receiver, at stage "1", the refrigerant is liquefied and split into the medium temperature (MT) string and the low temperature (LT) string, where expansion valves drops the pressure to the desired saturation temperature. The evaporators are controlled with valves using either hysteresis (open/close) or modulating (continues open) control -- valve $i$ has a corresponding valve constant, denoted $A_i$,. After the evaporators at stage "3a" and "3b", the refrigerant is superheated to avoid any droplets from entering the compressor. At stage "4a", "4b" and "5", after the low pressure compressor rack, the pressure is the same, but the enthalpy varies as the MT string and by-pass (bp) string from the receiver connects. The refrigerant now enters the high pressure compressor rack and continues through the condenser to a sub-cooled state throttled to stage ”8” and split in a liquid and a gas fraction  -- and the cycle repeats. Note, at higher ambient temperatures the refrigerant does not condense, but the gas is throttled and this result in a lower liquid and a higher gas fraction at “8”.

This research focus on modelling the evaporators, hence anything between stage "6" and "8" will not be discussed further. 


\section{Methodology}

In this section, first, under the assumption that there are no transient dynamics in processes, the steps in setting up a linear regression model for estimation of the valve constant are described, and second, the applied OLS estimation technique is presented, and finally to include linear dynamics an ARMAX model \cite{madsen2007time} is presented.

The valve constant $A_i$ is used to determine the refrigerant mass flow through evaporator $i$ by
\begin{align}\label{eq:mass_cab}
    \dot{m}_{\text{cab},i,t} = \sqrt{(P_{\text{rec},t} - P_{\text{e},i,t} ) \rho_{\text{liq},t}  } \lambda_{i,t} A_i,
\end{align}
where $P_{\text{rec},t}$ is the receiver pressure at time $t$ and $\rho_{\text{liq},t}$ is the density of the liquefied refrigerant, which is found as a function of $P_{\text{rec},t}$ using CoolProp \cite{coolprop}. For the $i$'th cabinet $P_{\text{e},i,t}$ is the evaporator pressure at time $t$, $\lambda_{i,t}$ is the opening degree of the valve at time $t$, given as a value between 0 and 1 and is controlled either using hysteresis (open/close) or modular (continues open) control. Hence, the valve constant, $A_i$, is defined as an area equivalent to the area of the valve opening when the valve is fully open.

The mass balance at stage "4a" (Figure \ref{fig:System}) can be written as
\begin{align}\label{eq:mass_balance}
    \dot{m}_{\text{MT,comp,t}} - \dot{m}_{\text{bp},t} = \sum_{i=1}^{n_{\text{LT}}} \dot{m}_{\text{cab},i,t} + \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} \dot{m}_{\text{cab},i,t},
\end{align}
where the $\dot{m}_{\text{MT,comp},t}$ is the mass flow going through the medium pressure (temperature) compressor at time $t$ and $\dot{m}_{\text{bp},t}$ is the by-pass mass flow entering from the receiver at time $t$. The right side mass flows are simply the sum of all the mass flows through the LT and MT cabinets, where $n_{\text{LT}}$ and $n_{\text{MT}}$ are the total number of LT and MT cabinets, respectively.

The mass flows on the left side of Equation \ref{eq:mass_balance} are calculated by
\begin{align}\label{eq:mass_MT}
    \dot{m}_{\text{MT,comp},t} = f_{\text{comp},t} \eta_{\text{vol}}  V_\text{s} \rho_{\text{gas}},
\end{align}
where f$_\text{comp}$ is the virtual compressor frequency (load as percentage of maximum capacity) at time $t$, $\eta_{\text{vol}} \sim 0.9 $, $V_\text{s}$ is the displacement volume which is specified for the compressor, and finally the mass flow from the by-pass valve is calculated by
\begin{align}\label{eq:mass_bp}
    \dot{m}_{\text{bp},t} = Q_t (h_{\text{gc},t}, P_{\text{rec},t})\, \dot{m}_{\text{MT,comp},t}.
\end{align}
where $Q_t$ is the gas quality of the refrigerant from the by-pass valve as a function of the enthalpy in the gas cooler, $h_{\text{gc},t}$, and the receiver pressure $P_{\text{rec},t}$ at time $t$.

In order to set up the a linear regression model with the valve constants as coefficients, we let
\begin{align}
x_{i,t} =  \sqrt{(P_{\text{rec},t} - P_{\text{e},i,t}) \rho_{\text{liquid},t}} \lambda_{i,t},
\end{align}
such that the right side of Equation \ref{eq:mass_balance} can be rewritten as
\begin{align}
  \sum_{i=1}^{n_{\text{LT}}} x_{i,t} A_i + \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} x_{i,t} A_i,
\end{align}
and
\begin{align}
    y_t = \dot{m}_{\text{MT,comp},t} - \dot{m}_{\text{bp},t}.
\end{align}
\begin{comment}
From the overview in Figure \ref{fig:System}, it is clear that 

 For the MT cabinets,  we can setup the following mass balance
\begin{align}
    \dot{m}_{\text{MT,comp}} - \dot{m}_{\text{LT,comp}} - \dot{m}_{\text{bp}} = \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} \dot{m}_{i} = \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} x_{i} A_i ,
\end{align}
where $n_{\text{MT}}$ is the number of MT cabinets. We can calculate the mass flow from the by-pass valve as
\begin{align}
    \dot{m}_{\text{bp}} = Q(h_{\text{gc}}, P_{\text{rec}}) \dot{m}_{\text{MT,comp}},
\end{align}

where $Q$ is the gas quality of the refrigerant from the by-pass valve as a function of the enthalpy in the gas cooler, $h_{\text{gc}}$, and the receiver pressure $P_\text{rec}$. This can be combined to the expression
\begin{align}\label{eq:mass_MT}
    \dot{m}_{\text{MT,comp}} (1- Q(h_{\text{gc}}, P_{\text{rec}})) - \dot{m}_{\text{LT,comp}} &= \sum_{i=n_{\text{LT}+1} 1}^{n_{\text{MT}}} x_i A_i ,
\end{align}

%\begin{figure}
%	\centering
%		\includegraphics[scale=.2]{Figures/od_cor_pow.png}
%	\caption{Opening degree of the  }
%	\label{fig:correlation_power}
%\end{figure}


\begin{align}\label{eq:final}
    \dot{m}_{\text{MT,comp}} (1- Q(h_{gc}, P_{\text{rec}})) &= \sum_{i=1}^{n_{\text{MT}}} x_i A_i + \sum_{i=n_{\text{MT}} + 1}^{n_{\text{LT}}} x_i A_i\nonumber 
\end{align}.
\end{comment}
The linear regression model can by set up by
\begin{align}
    \boldsymbol{y} &= \begin{bmatrix}
                        y_{1} & y_{2} & \cdots &  y_{n}
                    \end{bmatrix}^T \nonumber \\
    \boldsymbol{x} &= \begin{bmatrix}
                        x_{1,1} & x_{2,1} &  \cdots & x_{n_\text{V},1} \\
                        x_{1,2} & x_{2,2} & \cdots & x_{n_\text{V},2}\\
                        \vdots & \vdots &   \ddots & \vdots \\
                        x_{1,n} & x_{2,n} & \cdots & x_{n_\text{V},n} 
                    \end{bmatrix}\\
    \boldsymbol{\beta} &= \begin{bmatrix}
                        A_{1} & A_{2} &  \cdots & A_{n_V} 
                    \end{bmatrix}^T ,
                    \nonumber 
\end{align}
where $n$ is the number of observations and $n_\text{V} = n_{\text{MT}} + n_{\text{LT}}$, and thus can be written as
\begin{align}
    \boldsymbol{Y} = \boldsymbol{x}\boldsymbol{\beta} + \boldsymbol{\epsilon},
\end{align}
where the errors are random variables in the vector  
\begin{align}
  \boldsymbol{\epsilon} = \begin{bmatrix}
                        \epsilon_{1} & \epsilon_{2} & \cdots &  \epsilon_{n},
                    \end{bmatrix}^T
\end{align}
which must fulfill $\epsilon_t \sim N(0,\sigma^2 I)$ and i.i.d. Note, that $\boldsymbol{Y}$ is capital, since it is the model output and thus a vector of random variables.


The parameter vector $\boldsymbol{\beta}$ can be estimated from the OLS regression that minimize
\begin{align}
S(\boldsymbol{\beta}) =  ||\boldsymbol{Y} - \boldsymbol{x}\boldsymbol{\beta}||^2 
\end{align}
which has the OLS solution
\begin{align}
\hat{\boldsymbol{\beta}} = (\boldsymbol{x}^T \boldsymbol{x})^{-1} \boldsymbol{x}^T \boldsymbol{y}.\label{eq:ols}
\end{align}

Furthermore, modelling time series variables with a linear regression model will, if there are any dynamics present, lead to auto-correlation of the errors. This violates the assumption of i.i.d and consequently, the coefficient estimates can be biased and statistics not valid. Thus, to account for this, we will consider an ARMAX model. Using the back-shift operator, $B$, this model can be written as
\begin{equation}
    Y_t = \boldsymbol{x}_t\boldsymbol{\beta} +  \frac{\theta(B)}{ \phi(B)} \epsilon_t
\end{equation}
where $\theta(B) = 1 + \theta_1 B^1 + ... + \theta_q B^q $ and $\phi(B) = 1 + \phi_1 B^1 + ... + \phi_p B^p$. %% $p$ is the number of lags in $Y$ and $\mathbf{x}$ (AR part), $q$ is the number of lags in $\epsilon$ and $d$ is the order of differentiating.
 The model is refered to as an ARMAX\textsubscript{p,q} model, where parameters $p$ and $q$ determines the order of the AR and MA part, respectively. Note, that there are no lags in input variable, $x_t$, in this formulation, hence it is not a full ARMAX model since it is constrained to a model order of the input polynomial set to zero, i.e.\ $s=0$ according to \cite{TSA}. For the parameter estimation, the \textsf{R} function \texttt{arimax} from the \texttt{TSA} package is used. It is estimating the parameters using based the maximum likelihood method.
\begin{comment}


\begin{equation}
    Y_{t} = \boldsymbol{x}_t\mathbf{\beta} + \epsilon_{t}  + \theta_1 \epsilon_{t-1} + \ldots + \theta_q \epsilon_{t-q} - \phi_1 Y_{t-1} - \ldots - \phi_p Y_{t-p} ,
\end{equation}

Considering an AR model the prediction errors are obtained as
\begin{equation} \label{eq:arima_pred}
    y_{t+h}-\hat{Y}_{t+h|t} = \beta \boldsymbol{x_t} + \epsilon_{t+h}   + \theta_1\epsilon_{t-1+h} + \ldots + \theta_{h-1} \epsilon_{t+1} .
\end{equation}
\end{comment}











\begin{figure*}[t]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/day_chart.pdf}
    \caption{$x_{i,t}$ of the cooling room MT$_2$ the 29th of October 2013.}\label{fig:night}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/Spectrums.pdf}
    \caption{The frequency spectrum for each of the evaporators.}\label{fig:specs}
  \end{minipage}
\end{figure*}


\section{Case Study}\label{sec:data}
\subsection{Data and sampling time}
The data used consists of 1-minute time series covering an eight months period from November 2013 to June 2014. The values for one cabinet during one night is illustrated in Figure \ref{fig:night}. If the raw 1-minute data is used, a lot of redundant high frequency dynamics are present in the data that will lead to a poor model with high auto correlation. Thus we need to explore the impact of the sampling time on the model.
From the frequency spectrum shown in Figure \ref{fig:specs} we observe that most of the cabinets have a clear peak. We can extract the inverse frequency at the peak for each cabinet -- that is the most often occurring cycle time for the valve opening. The peak cycle times identified are listed in Table \ref{tab:frequencies}. Note, cabinet MT$_7$ has an extremely flat curve compared to all the other evaporators, hence its 14 min. cycle time is not as significant. This is because it uses modulating control (continuously valve opening) thus it has no clear peak in the frequency spectrum. Furthermore, it is noticed that MT$_1$ has the largest cycle time of 83 minutes. However, its spectrum peak is low compared to the other evaporators -- it is a booster evaporator for MT$_2$ (they are both located in the refrigeration room) and continuously supplies the cooling that MT$_2$ cannot. The rest of the evaporators have cycles varying from 20 min. to 40 min., where MT$_3$, MT$_4$ and MT$_5$ are clustered around 40 min. -- these are three different evaporators in the same cooling cabinet. For a good model, we will need to have at least, and ideally, two measurements for each cycle (one open and one closed). Because the evaporators have such different cycle times, there is no sampling time that will fit all the evaporators optimally. For instance, a 20-minute sampling time is best for MT$_3$, MT$_4$ and MT$_5$, whereas a 10-minute sampling time is best for MT$_6$, LT$_2$ and LT$_3$. For this study, we will therefore examine sampling time in the range of 1 min. to 30 min. The re-sampling from 1-minute sampling time to higher sampling times is carried out by averaging in the time periods, such that aliasing is avoided and a better signal-to-noise ratio in the re-sampled data is obtained \cite{TSA}. 

In order to evaluate if the estimated valve constants, $A_i$, have realistic values they are compared to the specified valve constants \cite{Fredslund} (see Table \ref{tab:danfoss_valves}).


\begin{comment}

The 10-minute sampling time data is illustrated in Figure \ref{fig:timeseries}. Notably, we have two large gaps of missing data in November and December 2013, however, this will not affect the results for linear regression. Examining closely the smoothed average curve for $\boldsymbol{y}$, it begins to increase in May, suggesting some seasonality with increased load during the summer. Furthermore, there is a change in the operation of LT$_2$ around February 2014. Prior, there was larger fluctuation and the regulation was forcing a thermostat cutout often, which is just the normal operation of a hysteresis control when the temperature reaches the cutout temperature. After February, the cabinet never reaches the cutout temperature and the valve is triggered by the pressure control instead.  
\end{comment}
\begin{table}[htbp]
\small
  \centering
    \begin{tabular}{p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1cm} }
    MT$_1$  & MT$_2$  & MT$_3$  & MT$_4$  & MT$_5$   & MT$_6$   \\
    \hline 
    83.17 & 32.19 & 39.92 & 41.58 & 41.58 & 21.23 \\[10pt]
     MT$_7$  & LT$_1$  & LT$_2$  & LT$_3$  & LT$_4$  & \\
     \hline
     14.68 & 31.19 & 25.59 & 20.37 & 30.24 &  


\end{tabular}%
\caption{The dominant inverse frequency for each cabinet in minutes.}\label{tab:frequencies}
\end{table}%



\begin{figure*}[t]
	\centering
		\includegraphics[scale=.35]{Figures/timeseries2.pdf}
	\caption{Daily averages of $x_{i,t}$ for each cabinet and $\mathbf{Y}$.}
	\label{fig:timeseries}
\end{figure*}
\begin{figure*}[t]
  \centering
    \includegraphics[scale=.35]{Figures/ts_results_lm.pdf}
	\caption{Estimated valve constant, $A_i$, for evaporator MT$_i$ as a function of the sampling time using all the data -- November 2013 to June 2014.}\label{fig:res}
\end{figure*}


%From Equation \ref{eq:mass_MT}, it is claimed that the variable $\boldsymbol{X}$ is correlated to the mass flow from the MT evaporators. This is confirmed in Figure \ref{fig:corr_plot} -- the top line in the scheme shows the correlation between the mass flow and $x$ for each cabinet. The color indicates the size of the valve -- the darker the blue the larger the valve. This genuinely tends to hold true according to actual valve constants -- see Appendix \ref{Appendix:Actual_valve_sizes}. 

The operation of evaporators within the same cabinet is obviously quite similar, thus correlations might occur -- this can be crucial for the model, as this can lead to problems with co-linearity in the estimation. When this happens the condition number of the matrix $\mathbf{X}$ is lowered, making the determinant of it close to zero, and thus inverting it results in large numerical errors, see Equation \ref{eq:ols}. However, in the present case the co-linearity was not an issue (generally, a correlation coefficient $>0.7$ indicates co-linearity \citep{Dormann} ). To confirm further, the Variance Inflation Factor (VIF) is a widely used tool -- a variant of stepwise regression used to detect multi co-linearity. A VIF less than 10 is an acceptable level \citep{Hair}, in present case the VIF was less than 2.


%\begin{figure}
%	\centering
%		\includegraphics[scale=0.5]{Figures/cor_valves.pdf}
%	\caption{Pearson correlation plot of $\boldsymbol{X}$ and the mass flow from the MT evaporators}
%	\label{fig:corr_plot}
%\end{figure}



==> Valve Estimation part 1 (1)/Chapters/Methodology2.tex <==
\section{The system}
The refrigeration system under study is illustrated in Figure \ref{fig:System}. Temperature and pressure measurements are accessible at all numbered points on the figure. After the receiver, at stage "1", the refrigerant is liquefied and split into the medium temperature (MT) string and the low temperature (LT) string, where expansion valves drops the pressure to the desired saturation temperature. The evaporators are controlled with valves using either hysteresis (open/close) or modulus (continues open) control - valve $i$ has a corresponding valve constant, denoted $A_i$. After the evaporators at stage "3a" and "3b", the refrigerant is super heated to avoid any droplets from entering the compressor. At stage "4a", "4b" and "5", after the low pressure compressor rack, the pressure is the same, but the enthalpy varies as the MT string and bypass (bp) string from the receiver connects. The refrigerant now enters the high pressure compressor rack and continues through the the condenser to a sub-cooled state at stage "8" - and the cycle repeats.

This research focus on modelling the evaporators, hence anything between stage "6" and "8" will not be discussed further. 

\begin{figure}
	\centering
		\includegraphics[scale=.2]{Figures/system_diagram.png}
	\caption{Exemplifying flow sheet of supermarket CO\textsubscript{2} refrigeration system. The valve constant for evaporator $i$ is denoted with $A_i$. $n_{\text{MT}}$ and $n_{\text{LT}}$ are the number of Medium -and Low Temperature evaporators respectively. }
	\label{fig:System}
\end{figure}



\section{Methodology}

\subsection{Method 1 - Valve estimation with known $V_s$}
The valve constants are used to determine the refrigerant mass flow through the evaporator $i$ from
\begin{align}
    \dot{m}_{\text{cab},i} = \sqrt{(P_{\text{rec}} - P_{e,i} ) \rho_{\text{liquid}}  } \lambda_i A_i ,
\end{align}
where $P_\text{rec}$ is the receiver pressure, $P_{\text{e},i}$ is the evaporator pressure for cabinet $i$, $\rho_{\text{liquid}}$ is the density of the liquefied refrigerant and $A$ is the valve constant. The opening degree of the valve of cabinet $i$, $\lambda_i$, is a number between 0 and 1 and is controlled either using hysteresis (open/close) or modular (continues open) control - this control parameter is highly correlated with the power load of the compressors - which of course links to the mass flow through the compressors. This mass flow can be expressed as
\begin{align}\label{eq:mass_comp}
    \dot{m} = \text{CAP} \eta_{\text{vol}} \cdot V_s \rho_{gas},
\end{align}
where $\eta_{\text{vol}, LT} \sim 0.8 $ and $\eta_{\text{vol}, MT} \sim 0.9 $. The displacement volume, $V_s$, can be obtained from the compressor information plate. From the overview in Figure \ref{fig:System}, it is clear that 
\begin{align}\label{eq:mass_LT}
    \dot{m}_{\text{LT,comp}} = \sum_{i=1}^{n_{\text{LT}}} \dot{m}_{\text{i}} = \sum_{i=1}^{n_{\text{LT}}} x_i A_i ,
\end{align}
where $n_{\text{LT}}$ is the total number of LT cabinets and $$x =  \sqrt{(P_{\text{rec}} - P_e ) \rho_{\text{liquid}}} \lambda $$
 For the MT cabinets,  we can setup the following mass balance
\begin{align}
    \dot{m}_{\text{MT,comp}} - \dot{m}_{\text{LT,comp}} - \dot{m}_{\text{bp}} = \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} \dot{m}_{i} = \sum_{i=n_{\text{LT}}+1}^{n_{\text{MT}}} x_{i} A_i ,
\end{align}
where $n_{\text{MT}}$ is the number of MT cabinets. We can calculate the mass flow from the by-pass valve as
\begin{align}
    \dot{m}_{\text{bp}} = Q(h_{\text{gc}}, P_{\text{rec}})\cdot \dot{m}_{\text{MT,comp}},
\end{align}

where $Q$ is the gas quality of the refrigerant from the by-pass valve as a function of the enthalpy in the gas cooler, $h_{\text{gc}}$, and the receiver pressure $P_\text{rec}$. This can be combined to the expression
\begin{align}\label{eq:mass_MT}
    \dot{m}_{\text{MT,comp}} (1- Q(h_{\text{gc}}, P_{\text{rec}})) - \dot{m}_{\text{LT,comp}} &= \sum_{i=n_{\text{LT}+1} 1}^{n_{\text{MT}}} x_i A_i ,
\end{align}

%\begin{figure}
%	\centering
%		\includegraphics[scale=.2]{Figures/od_cor_pow.png}
%	\caption{Opening degree of the  }
%	\label{fig:correlation_power}
%\end{figure}

Furthermore, by substituting Equation \ref{eq:mass_LT} into Equation \ref{eq:mass_MT}, the need for calculating the $\dot{m}_{\text{LT,comp}}$ is eliminated and it simplifies to

\begin{align}\label{eq:final}
    \dot{m}_{\text{MT,comp}} (1- Q(h_{gc}, P_{\text{rec}})) &= \sum_{i=1}^{n_{\text{MT}}} x_i A_i + \sum_{i=n_{\text{MT}} + 1}^{n_{\text{LT}}} x_i A_i\nonumber 
\end{align}.

Let $ y_t = \dot{m}_{\text{MT, comp},t} (1- Q(h_{\text{gc},t}, P_\text{rec},t)) $, then 
\begin{align}
    \boldsymbol{y} &= \begin{bmatrix}
                        y_{1} & y_{2} &  y_{n}
                    \end{bmatrix} \nonumber \\
    \boldsymbol{X} &= \begin{bmatrix}
                        x_{1,1} & x_{2,1} &  x_{n_V,1} \\
                        x_{1,2} & x_{2,2} & x_{n_V,2}\\
                        x_{1,n} & x_{2,n} & x_{n_V,n} 
                    \end{bmatrix}\nonumber \\
    \boldsymbol{\beta} &= \begin{bmatrix}
                        A_{1} & A_{2} &  A_{n_V} 
                    \end{bmatrix} \nonumber 
\end{align}
,
where $n$ is the number of observations and $n_V = n_{\text{MT}} + n_{\text{LT}}$.
 
And finally, we can write the linear regression model:
\begin{align}
    \boldsymbol{y} &= \boldsymbol{X}\boldsymbol{\beta} + \boldsymbol{\epsilon}, \\
    \text{for} \; \boldsymbol{\epsilon} &\sim N(0,\sigma^2 I) \; \text{and i.i.d},  \nonumber
\end{align}

Then $\boldsymbol{\beta}$ can be estimated from the least square regression that minimize:
\begin{align}
S(\boldsymbol{\beta}) =  ||\boldsymbol{y} - \boldsymbol{X}\boldsymbol{\beta}||^2 
\end{align}
and we obtain the ordinary least-squares solution
\begin{align}
\boldsymbol{\beta} = (\boldsymbol{X}^T \boldsymbol{X})^{-1} \boldsymbol{X}^T \boldsymbol{y}.\label{eq:ols}
\end{align}

% Since the outdoor temperature affects the efficiency of refrigeration systems, it can be beneficial to implement that into the model, e.g. $\boldsymbol{\beta} = [A_1,...,A_{n_V}, A_{T}]$, where $A_{T}$ is the coefficient for the temperature. % Furthermore, it is expected that operation during the day will lead to larger errors due to disturbances. 
\begin{figure*}[t]
	\centering
		\includegraphics[scale=.4]{Figures/optim.png}
	\caption{Optimization function}
	\label{fig:algorithm}
\end{figure*}
\subsection{Part 2 - Valve estimation with $V_{\text{s}}$ unknown} \label{sec:unknown_v}

The compressor stroke volume, $V_{\text{s}}$, is not always easily accessible thus for automatic implementation on a large scale, a valve estimation methodology with $V_s$ unknown is required. With knowledge about the types of valves there possibly can be in the system - see Table \ref{tab:danfoss_valves} in Appendix \ref{Appendix:Actual_valve_sizes} - a novel algorithm was developed, using K-means for clustering the estimated valve constants $\mathbf{A}$. Figure \ref{fig:algorithm} illustrates part of the algorithm. 

\begin{itemize}
    \item We have a function with two inputs:
    \begin{itemize}
        \item The MT compressor stroke volume $V_{\text{s}}$
        \item An initial guess of the different types of valve we have in the system - we call that $a$.
    \end{itemize}
    \item First we estimate the model coefficients, $\hat{\boldsymbol{\beta}}$, from Equation \ref{eq:ols}.  
    \item Then we apply k-means to $ \hat{\boldsymbol{\beta}}$ e.g. each $\hat{\beta}_i$ is assigned to cluster $S_i$ by minimizing:
    
    $$
    \argmin_S \sum_{i=1}^k \sum_{\boldsymbol{x} \in S_i} \norm{\boldsymbol{x} - \boldsymbol{C_i}}^2,
    $$
    where $\boldsymbol{C_i}$ is the mean of cluster $i$:
    \begin{align}
    C_i = \frac{1}{S_i^{(t)}} \sum_{A_j \in S_i^{(t)}} A_j
    \end{align}
\end{itemize}

% $f(V_{\text{s}})$ refers to Equation \ref{eq:final}, where  $\dot{m}_{MT}$ is a function of $V_s$ (see Eq. \ref{eq:mass_comp}). The illustration is a function with two inputs; the compressor stroke volume, $V_s$, and an initial guess of $\mathbf{a}$ (the kind of valves that exist in the system). The output is a Root Mean Squared Error of $\epsilon$. 
%First, we will get an estimate of the valve constants $\mathbf{A}$ from $f(V_s)$. Then we apply k-means to $\mathbf{A}$ e.g. each $A_i$ is assigned to cluster $S_i$ as:
%\begin{align}
%    S_i^{(t)} = A_p : \norm{A_p - C_i^{(t)} }^2 \leq \norm{A_p - C_j^{(t)} }^2 \;\; \forall, 1 \leq j \leq k
%\end{align}
%where $k$ is the number of valve constants in $\mathbf{a}$ and $\mathbf{C}$ is the cluster means:





$\boldsymbol{C}$ and $\boldsymbol{a}$ are sorted vectors from smallest to largest so that we get the error
$
    \epsilon_1 = \ln{\boldsymbol{C}} - \ln{\boldsymbol{a}}
$. 
At last, we get the Root Mean Squared Error output of the function, referred to as $E_1$:
\begin{align}\label{eq:E_1}
    E_1 = \frac{\sqrt{\sum_{i=1}^{N_{\epsilon_1}} \epsilon_{1,i}^2}}{N_{\epsilon_1}},
\end{align}
where $N_{\epsilon}$ is the length of $\epsilon$.

For the optimization, we assume $\boldsymbol{a}$ is known and use the one dimensional "Brent" optimization algorithm to find the $V_{\text{s}}$ that minimizes the $E_1$.
With 7 different types of valves, we have 127 different combinations of $\boldsymbol{a}$ thus the above algorithm is not enough on its own. By running the algorithm on all the combinations, we can investigate the errors and pick out the combination that produces the best model. For the error estimates, we use $E_1$ and the following:
\begin{align}\label{eq:E_2}
    E_2 = \frac{1}{n_V} \sum_{i=1}^k \sum_{\hat{\beta}_j \in S_i} (\ln{C_i} - \ln{\hat{\beta}_j})^2,
\end{align}
%where
%\begin{align}
%    \epsilon_{2,j} =   \ln{C_i} -  \ln{A_j}; \quad  A_j \in S_i^{(t)}\nonumber
%\end{align}

$E_2$ is thus the cluster uncertainty of $\boldsymbol{C}$.

% Furthermore, we are interested in a normally distributed $E_1$, which can be indicated by the skewness:

%\begin{align}
%    \text{Skewness} &= 3*(C_{E_1} - \text{median}_{E_1}) / \sigma_{E_1} \label{eq:skewness}
%\end{align}
%A large skewness means that at least one of the estimates in $\mathbf{C}$ stands out from the rest, indicating one too many or one too few valves in $a$.
%A last criteria is the correlation between $\mathbf{C}$ and $ \mathbf{a}$:
%\begin{align}
%    \rho &=     \frac{\text{cov}(\ln{\mathbf{C}} , \ln{\mathbf{a}})}{\sigma_C \sigma_a}. \label{eq:rho}
%\end{align}

%The closer $\rho$ is to 1, the more correct are the internal "jumps" between the valve sizes e.g. $a_j - a_i$ is similar to $C_j - C_i$. 




\subsection{Data}the data stretch approximately eight months from November 2013 to June 2014
The data is available in 1 minute values stretching approximately eight months from November 2013 to June 2014 and is illustrated for one cabinet during one night in Figure \ref{fig:night} (left plot). If we use the raw 1-minute data, we will experience a lot of redundant noise that will lead to a bad model with auto correlation. Thus we need to find the best data resolution for the model. One way is to find the lowest resolution that removes all significant auto-correlation from the model. In this case, 20 minute data is found to be the optimal resolution.

 


\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{Figures/night_operation.pdf}
    \caption{left plot: $x$ of cabinet 20A (freezing room) the 26th of October 2013. Right plot: The frequency spectrum for 20A.}
    \label{fig:night}
\end{figure*}


\begin{figure*}[t]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/timeseries.png}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figures/timeseries2.png}
  \end{minipage}
  \caption{Daily averages of the mass flow through the MT evaporators, $\mathbf{Y}$, and $\mathbf{X}$ for all the cabinets.}\label{fig:timeseries}
\end{figure*}


%From Equation \ref{eq:mass_MT}, it is claimed that the variable $\boldsymbol{X}$ is correlated to the mass flow from the MT evaporators. This is confirmed in Figure \ref{fig:corr_plot} - the top line in the scheme shows the correlation between the mass flow and $x$ for each cabinet. The color indicates the size of the valve - the darker the blue the larger the valve. This genuinely tends to hold true according to actual valve constants - see Appendix \ref{Appendix:Actual_valve_sizes}. 
Some of the cabinets are connected on the same string e.g. 40A, 40B and 40C - see Appendix \ref{Appendix:structure} for the cabinet structure. The operation of these cabinets is therefore quite similar and correlation might occur - this can be crucial for the model, as this can lead to co-linearity. When this happens the condition number of the matrix $\mathbf{X}$ is lowered, making the determinant of it close to zero, and thus inverting it results in large numerical errors - see Equation \ref{eq:ols}. However, in this case co-linearity is not an issue (generally, a correlation coefficient $>0.7$ indicates co-linearity \cite{Dormann} ). To confirm further, the Variance Inflation Factor (VIF) is a widely uesd tool - a variant of stepwise regression used to detect multi co-linearity. A VIF less than 10 is an acceptable level \cite{Hair} - in this case, the VIF is less than 2.


\begin{figure}
	\centering
		\includegraphics[scale=0.5]{Figures/cor_valves.pdf}
	\caption{Pearson correlation plot of $\boldsymbol{X}$ and the mass flow from the MT evaporators}
	\label{fig:corr_plot}
\end{figure}



==> Valve Estimation part 1 (1)/Chapters/Results.tex <==
\section{Results}

As discussed in Section \ref{sec:data}, the sampling time potentially impacts the estimated parameters, thus this was investigated and the result of this is presented in this section -- and how the suggested method for determining the optimal time resolution, identified based on their cycle frequencies, see Figure \ref{fig:specs} and Table \ref{tab:frequencies}, lead to reliable estimates. First the results of applying the linear regression model are presented and thereafter the results from the ARMAX model.

\subsection{Linear Regression Model}

The estimated valve constants are presented as function of the sampling time in Figure \ref{fig:res}. In each figure the red line marks the specified valve constant (see Table \ref{tab:danfoss_valves}), the green line marks the identified optimal sampling time and the black line is the valve constant estimates (with the 95\% CI) vs. the sampling time from 1 min. to 30 min.. The estimates clearly vary with the sampling time, however the estimator converge to a constant level with higher sampling times in most cases. Both the estimates for MT$_2$ and MT$_5$ seem to decrease after the sampling time exceeds their respective optimal sampling time. Furthermore, at low sampling times (< 10 minutes) the estimates are typically diverging. By observing the Auto Correlation Function (ACF) of the residuals for the 1-minute model and the 15-minute model presented in Figure \ref{fig:acf} (top left and top right plot respectively), there is clearly significant auto-correlation for both models, which indicates the need for modelling dynamics with an ARMAX model.
\begin{figure*}
 \includegraphics[scale=0.75]{Figures/acf_all.pdf}
	\caption{Auto Correlation functions (ACF) for the linear regression models and ARMAX models using 1 minute and 15 minute sampling time.}\label{fig:acf}
\end{figure*}

\begin{table}[htbp]
\small
  \centering
    \begin{tabular}{l c c}
    Cabinet & Valve  &  $A [\sqrt{10} m^2]$ \\

    MT$_1$ & AKV 10-3  & 0.58765 \\
    MT$_2$ & AKV 10-5 &  1.48523\\
    MT$_3$ & AKV 10-4 &  0.94185 \\
    MT$_4$ & AKV 10-5 &  1.48523\\
    MT$_5$ & AKV 10-5 &  1.48523\\
    MT$_6$ & AKV 10-5 &  1.48523 \\
    MT$_7$ & AKV 10-2 &  0.37191\\
    LT$_1$ & AKV 10-3 &  0.58765\\
    LT$_2$ & AKV 10-2 &  0.37191\\
    LT$_3$ & AKV 10-2 &  0.37191\\
    LT$_4$ & AKV 10-2 &  0.37191



\end{tabular}%
\caption{Valves installed in Fakta Otterup and their valve constants $A$ - derived from a previous study \cite{Fredslund} }\label{tab:danfoss_valves}
\end{table}%

\subsection{ARMAX Model}

The ACF of the linear regression model using 1-minute sampling time, see Figure \ref{fig:acf} top left plot, shows seasonality caused by hysteresis control with roughly 15 lags between the wave peaks. Now, consider the ACF of the 15-minute sampling time model (Figure \ref{fig:acf}, top right), there is a large negative correlation to lag 1, which implies the need for a moving average term. The positive correlation of lag 4 implies the need for auto-regressive terms.
An ARMAX$_{4,1}$ model removed all auto-correlation in the 15 min. sampling time model (Figure \ref{fig:acf}, bottom right). In this study, an ARMAX$_{4,1}$ will be used for all sampling times, though the best ARMAX fit may be different for other sampling times.
The 1-min. model still has some seasonal auto-correlation (Figure \ref{fig:acf}, bottom left), but it is much improved. Considering the resulting valve constant estimates, presented in Figure \ref{fig:res_arimax}, firstly, it is found that the CIs are much more narrow compared with the CIs for the linear regression model. Secondly, the estimates vary with the sampling time and above a certain level the estimates converge.

\begin{figure*}[t]
  \centering
    \includegraphics[scale=.35]{Figures/ts_results_arimax.pdf}
	\caption{Estimated parameters as a function of the sampling time using all the data - November 2013 to June 2014.}\label{fig:res_arimax}
\end{figure*}



\begin{comment}
\begin{figure*}
  \centering
  \begin{minipage}[b]{0.45\textwidth}
   \includegraphics[scale=.35]{Figures/acfLM1.pdf}
	\caption{Linear regression model: Auto Correlation Function for the 1-minute model.  \newline resolution model.}\label{fig:acfLM1}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[scale=.35]{Figures/acfLM15.pdf}
	\caption{Linear regression model: Auto Correlation Function for the 15-minute model.  \newline resolution model.}\label{fig:acfLM15}
  \end{minipage}
\end{figure*}


\begin{figure*}
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[scale=.35]{Figures/acfARIMAX1.pdf}
	\caption{ARMAX model: Auto Correlation Function for the 1-minute model.  \newline resolution model.}\label{fig:acfARIMAX1}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[scale=.35]{Figures/acfARIMAX15.pdf}
	\caption{ARMAX model: Auto Correlation Function for the 15-minute model.  \newline resolution model.}\label{fig:acfARIMAX15}
  \end{minipage}
\end{figure*}
\end{comment}

==> Valve Estimation part 1 (1)/Figures/model.tex <==
%% Scaling the nodes
\tikzset{every node/.style={scale=\scaleTikz}}
%% The tikz
\begin{circuitikz}[xscale=\scaleTikz, yscale=\scaleTikz]
  %% Define variables to control size
  \def\x{2.3}    % x distance between nodes
  \def\y{3.3}    % y position of the diagram
  \def\ylab{4} % y position of the labels
  %% Set the coordinates
 \coordinate (Goods) at (0,0);
 \coordinate (R_goods) at ($(Goods)+(\x,0)$);
 \coordinate (Cabinet) at ($(R_goods)+(\x,0)$);
 \coordinate (R_c) at ($(Cabinet)+(\x,0)$);

 
 
 
  \coordinate (Floor) at (0,0);
  \coordinate (Heater) at ($(Floor)+(0.8*\x,0)$);
  \coordinate (SolarFloor) at ($(Heater)+(\x,0)$);
  \coordinate (Interior) at ($(SolarFloor)+(\x,0)$);
  \coordinate (SolarInterior) at ($(Interior)+(1.3*\x,0)$);
  %\coordinate (HeaterInterior) at ($(Interior)+(\x,0)$);
  \coordinate (WallLeft) at ($(SolarInterior)+(0.45*\x,0)$);
  \coordinate (Wall) at ($(WallLeft)+(0.8*\x,0)$);
  \coordinate (WallRight) at ($(Wall)+(0.8*\x,0)$);
  \coordinate (Ambient) at ($(WallRight)+(0.25*\x,0)$);
  %% Draw stuff
  \draw
  ($(3.15*\x,0)$) node[ground] {}
  % ($(6.15*\x,0)$) node[ground] {}

 % ($(Floor)+(0,4.5)$) -- ($(SolarFloor)+(0,4.5)$)
 % ($(Floor)+(0,6)$) -- ($(SolarFloor)+(0,6)$)
 
  %($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1)$)
  %($(Heater)+(\xoffset,1)$) to[I, l=$\Ph$] %($(Heater)+(\xoffset,\y)$);
 
  (Goods) -- (Ambient) % The bottom line
  %%($(Floor)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  ($(Goods)+(0,\y)$) -- ($(R_goods)+(0,\y)$) % The top line
   ($(Cabinet)+(0,\y)$) -- ($(R_c)+(0,\y)$); % The top line
%%($(R_c)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  % The top line

  %% The Floor
 \draw
  (Goods) to[C=$\Cg$, -*] ($(Goods)+(0,\y)$)
  {[anchor=south east] ($(Goods)+(0.2,\y)$) node {$\Tg$}};
  %% The Heater
%%  \def\xoffset{-0.25*\x}
%%  \draw
%%  ($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1.2)$)
%%  ($(Heater)+(\xoffset,1.2)$) to[I, l_=$(1-\Psi\n{h})\Ph$] %%($(Heater)+(\xoffset,\y)$);
  
  %% The Solar to floor
 %% \def\xoffset{0.1*\x}
 %% \draw
 %% ($(SolarFloor)+(\xoffset,0)$) to[I, l=$(1-\Psi\n{s}) %%\gA\Ps$]($(SolarFloor)+(\xoffset,\y-1.2)$)
 %% ($(SolarFloor)+(\xoffset,\y-1.2)$) -- %%($(SolarFloor)+(\xoffset,\y)$);
  %% Resistance
  \draw
  ($(R_goods)+(0,\y)$) to [R, l=$\Rg$] ($(Cabinet)+(0,\y)$);
  %% The Interior
  \draw
  (Cabinet) to[C=$\Cc$, -*] ($(Cabinet)+(0,\y)$)
  {[anchor=south east] ($(Cabinet)+(0.2,\y)$) node {$\Tc$}};
 \draw
  ($(R_c)+(0,\y)$) to [R, l=$\Rload$] ($(Ambient)+(0,\y)$);


  %% The Solar to interior
  \def\xoffset{0.1*\x}
  \draw
  %%($(Heater)+(\xoffset+5.5,0)$) -- ($(Heater)+(\xoffset+5.5,0.2)$)
  ($(Heater)+(\xoffset+5.5,0)$)
  to[I, l_=$ \frac{1}{\Rm } \Mr (\Tc-\Te)$] ($(Heater)+(\xoffset+5.5,\y)$);
  

%%  \def\xoffset{0*\x}
 %% \draw
 %% ($(SolarInterior)+(\xoffset+0.5,0)$) to[I, %%l=$\Psi\n{s}\gA\Ps$]($(SolarInterior)+(\xoffset+0.5,\y-1.2)$)
%%  ($(SolarInterior)+(\xoffset+0.5,\y-1.2)$) -- ($(SolarInterior)+(\xoffset+0.5,\y)$);
  %% The Wall
  %%\draw
 %% ($(WallLeft)+(0,\y)$) to [R, l=$\Riw$, -*] ($(Wall)+(0,\y)$)        
 %% ($(Wall)+(0,\y)$) to [R, l=$\Rwa$] ($(WallRight)+(0,\y)$)
 %% ($(WallRight)+(0,\y)$) -- ($(Ambient)+(0,\y)$)
 %% (Wall) to[C=$\Cw$, -] ($(Wall)+(0,\y)$)
 %% {[anchor=south east] ($(Wall)+(0.2,\y)$) node {$\Tw$}};
  %% The Ambient
  \draw
  [V, l=$\Ta$] ($(Ambient)+(0,\y)$) to ($(Ambient)+(0,0)$);
  %% The dashed lines
 %% \def\xoffset{0.22*\x}
 %% \draw
 %% [dashed] ($(SolarFloor)+(\xoffset*\x,-0.5)$) -- %%($(SolarFloor)+(\xoffset*\x,\y-0.4)$)  
%%  [dashed] ($(SolarFloor)+(\xoffset*\x,\ylab+0.2)$) -- ($(SolarFloor)+(\xoffset*\x,\ylab+1)$)  
%%  [dashed] ($(WallLeft)+(0.15,-0.5)$) -- ($(WallLeft)+(0.15,\ylab+1)$)  
%%  [dashed] ($(Ambient)+(-0.3*\x,-0.5)$) -- ($(Ambient)+(-0.3*\x,\ylab+1)$);
  %% The labels
 %% \draw
%%  {[anchor=south] ($(Heater)+(0.2,\ylab)$) node{\Large Floor}}
%%  {[anchor=south] ($(Interior)+(0.7*\x,\ylab)$) node{\Large Interior}}
%%  {[anchor=south] ($(Wall)+(0,\ylab)$) node{\Large Envelope}}
 %% {[anchor=south] ($(Ambient)+(0.2*\x,\ylab)$) node{\Large Ambient}};

\end{circuitikz}


==> Valve Estimation part 1 (1)/Figures/model_simple.tex <==
%% Scaling the nodes
\tikzset{every node/.style={scale=\scaleTikz}}
%% The tikz
\begin{circuitikz}[xscale=\scaleTikz, yscale=\scaleTikz]
  %% Define variables to control size
  \def\x{2.3}    % x distance between nodes
  \def\y{3.3}    % y position of the diagram
  \def\ylab{4} % y position of the labels
  %% Set the coordinates
 \coordinate (Goods) at (0,0);
 \coordinate (R_goods) at ($(Goods)+(\x,0)$);
 \coordinate (Cabinet) at ($(R_goods)+(\x,0)$);
 \coordinate (R_c) at ($(Cabinet)+(\x,0)$);

 
 
 
  \coordinate (Floor) at (0,0);
  \coordinate (Heater) at ($(Floor)+(0.8*\x,0)$);
  \coordinate (SolarFloor) at ($(Heater)+(\x,0)$);
  \coordinate (Interior) at ($(SolarFloor)+(\x,0)$);
  \coordinate (SolarInterior) at ($(Interior)+(1.3*\x,0)$);
  %\coordinate (HeaterInterior) at ($(Interior)+(\x,0)$);
  \coordinate (WallLeft) at ($(SolarInterior)+(0.45*\x,0)$);
  \coordinate (Wall) at ($(WallLeft)+(0.8*\x,0)$);
  \coordinate (WallRight) at ($(Wall)+(0.8*\x,0)$);
  \coordinate (Ambient) at ($(WallRight)+(0.25*\x,0)$);
  %% Draw stuff
  \draw
  ($(3.15*\x,0)$) node[ground] {}
  % ($(6.15*\x,0)$) node[ground] {}

 % ($(Floor)+(0,4.5)$) -- ($(SolarFloor)+(0,4.5)$)
 % ($(Floor)+(0,6)$) -- ($(SolarFloor)+(0,6)$)
 
  %($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1)$)
  %($(Heater)+(\xoffset,1)$) to[I, l=$\Ph$] %($(Heater)+(\xoffset,\y)$);
 
  (Cabinet) -- (Ambient) % The bottom line
  %%($(Floor)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  %%($(Goods)+(0,\y)$) -- ($(R_goods)+(0,\y)$) % The top line
   ($(Cabinet)+(0,\y)$) -- ($(R_c)+(0,\y)$); % The top line
%%($(R_c)+(0,\y)$) -- ($(Ambient)+(0,\y)$);
  % The top line

  %% The Floor
%% \draw
%%  (Goods) to[C=$\Cg$, -*] ($(Goods)+(0,\y)$)
%%  {[anchor=south east] ($(Goods)+(0.2,\y)$) node {$\Tg$}};
  %% The Heater
%%  \def\xoffset{-0.25*\x}
%%  \draw
%%  ($(Heater)+(\xoffset,0)$) -- ($(Heater)+(\xoffset,1.2)$)
%%  ($(Heater)+(\xoffset,1.2)$) to[I, l_=$(1-\Psi\n{h})\Ph$] %%($(Heater)+(\xoffset,\y)$);
  
  %% The Solar to floor
 %% \def\xoffset{0.1*\x}
 %% \draw
 %% ($(SolarFloor)+(\xoffset,0)$) to[I, l=$(1-\Psi\n{s}) %%\gA\Ps$]($(SolarFloor)+(\xoffset,\y-1.2)$)
 %% ($(SolarFloor)+(\xoffset,\y-1.2)$) -- %%($(SolarFloor)+(\xoffset,\y)$);
  %% Resistance
 %% \draw
%%  ($(R_goods)+(0,\y)$) to [R, l=$\Rg$] ($(Cabinet)+(0,\y)$);
  %% The Interior
  \draw
  (Cabinet) to[C=$\Cc$, -*] ($(Cabinet)+(0,\y)$)
  {[anchor=south east] ($(Cabinet)+(0.2,\y)$) node {$\Tc$}};
 \draw
  ($(R_c)+(0,\y)$) to [R, l=$\Rload$] ($(Ambient)+(0,\y)$);


  %% The Solar to interior
  \def\xoffset{0.1*\x}
  \draw
  %%($(Heater)+(\xoffset+5.5,0)$) -- ($(Heater)+(\xoffset+5.5,0.2)$)
  ($(Heater)+(\xoffset+5.5,0)$)
  to[I, l_=$ \frac{1}{\Rm }\Mr (\Tc-\Te)$] ($(Heater)+(\xoffset+5.5,\y)$);
  

%%  \def\xoffset{0*\x}
 %% \draw
 %% ($(SolarInterior)+(\xoffset+0.5,0)$) to[I, %%l=$\Psi\n{s}\gA\Ps$]($(SolarInterior)+(\xoffset+0.5,\y-1.2)$)
%%  ($(SolarInterior)+(\xoffset+0.5,\y-1.2)$) -- ($(SolarInterior)+(\xoffset+0.5,\y)$);
  %% The Wall
  %%\draw
 %% ($(WallLeft)+(0,\y)$) to [R, l=$\Riw$, -*] ($(Wall)+(0,\y)$)        
 %% ($(Wall)+(0,\y)$) to [R, l=$\Rwa$] ($(WallRight)+(0,\y)$)
 %% ($(WallRight)+(0,\y)$) -- ($(Ambient)+(0,\y)$)
 %% (Wall) to[C=$\Cw$, -] ($(Wall)+(0,\y)$)
 %% {[anchor=south east] ($(Wall)+(0.2,\y)$) node {$\Tw$}};
  %% The Ambient
  \draw
  [V, l=$\Ta$] ($(Ambient)+(0,\y)$) to ($(Ambient)+(0,0)$);
  %% The dashed lines
 %% \def\xoffset{0.22*\x}
 %% \draw
 %% [dashed] ($(SolarFloor)+(\xoffset*\x,-0.5)$) -- %%($(SolarFloor)+(\xoffset*\x,\y-0.4)$)  
%%  [dashed] ($(SolarFloor)+(\xoffset*\x,\ylab+0.2)$) -- ($(SolarFloor)+(\xoffset*\x,\ylab+1)$)  
%%  [dashed] ($(WallLeft)+(0.15,-0.5)$) -- ($(WallLeft)+(0.15,\ylab+1)$)  
%%  [dashed] ($(Ambient)+(-0.3*\x,-0.5)$) -- ($(Ambient)+(-0.3*\x,\ylab+1)$);
  %% The labels
 %% \draw
%%  {[anchor=south] ($(Heater)+(0.2,\ylab)$) node{\Large Floor}}
%%  {[anchor=south] ($(Interior)+(0.7*\x,\ylab)$) node{\Large Interior}}
%%  {[anchor=south] ($(Wall)+(0,\ylab)$) node{\Large Envelope}}
 %% {[anchor=south] ($(Ambient)+(0.2*\x,\ylab)$) node{\Large Ambient}};

\end{circuitikz}

